Pyramidal Denoising Diffusion Probabilistic Models

Recently, diffusion model have demonstrated impressive image generation performances, and have been extensively studied in various computer vision tasks. Unfortunately, training and evaluating diffusion models consume a lot of time and computational resources. To address this problem, here we present a novel pyramidal diffusion model that can generate high resolution images starting from much coarser resolution images using a {\em single} score function trained with a positional embedding. This enables a neural network to be much lighter and also enables time-efficient image generation without compromising its performances. Furthermore, we show that the proposed approach can be also efficiently used for multi-scale super-resolution problem using a single score function.

==> macros.tex <==
\newcommand{\ab}{{\boldsymbol a}}
\newcommand{\bb}{{\boldsymbol b}}
\newcommand{\p}{{\boldsymbol p}}
\newcommand{\x}{{\boldsymbol x}}
\newcommand{\y}{{\boldsymbol y}}
\newcommand{\z}{{\boldsymbol z}}
\newcommand{\ub}{{\boldsymbol u}}
\newcommand{\f}{{\boldsymbol f}}
\newcommand{\w}{{\boldsymbol w}}
\newcommand{\Ib}{{\boldsymbol I}}
\newcommand{\Jb}{{\boldsymbol J}}
\newcommand{\Ab}{{\boldsymbol A}}
\newcommand{\Db}{{\boldsymbol D}}
\newcommand{\Pb}{{\boldsymbol P}}
\newcommand{\Rb}{{\boldsymbol R}}
\newcommand{\Hb}{{\boldsymbol H}}
\newcommand{\Rd}{{\mathbb R}}
\newcommand{\Nd}{{\mathbb N}}
\newcommand{\Ed}{{\mathbb E}}
\newcommand{\Mc}{{\mathcal M}}
\newcommand{\Nc}{{\mathcal N}}
\newcommand{\Pc}{{\mathcal P}}

\newcommand{\epsilonb}{{\boldsymbol \epsilon}}

\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\rank}{rank}


\newtheorem{theorem}{\bf{Theorem}}
\newtheorem{lemma}{\bf{Lemma}}
\newtheorem{proposition}{\bf{Proposition}}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{\bf{Definition}}
\newtheorem{remark}{\bf{Remark}}
\newtheorem{example}{\bf{Example}}
\newtheorem{assumption}{Assumption}
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\def\code#1{\texttt{#1}}


% colors
\definecolor{trolleygrey}{rgb}{0.5, 0.5, 0.5}
\definecolor{darkpastelgreen}{rgb}{0.01, 0.75, 0.24}
\definecolor{darkpink}{rgb}{0.91, 0.33, 0.5}
\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}
\definecolor{americanrose}{rgb}{1.0, 0.01, 0.24}
